Deformation-based In-Context Learning for Point Cloud Understanding

Recent advances in point cloud In-Context Learning (ICL) have demonstrated strong multitask capabilities. Existing approaches typically adopt a Masked Point Modeling (MPM)-based paradigm for point cloud ICL. However, MPM-based methods directly predict the target point cloud from masked tokens without leveraging geometric priors, requiring the model to infer spatial structure and geometric details solely from token-level correlations via transformers. Additionally, these methods suffer from a training-inference objective mismatch, as the model learns to predict the target point cloud using target-side information that is unavailable at inference time. To address these challenges, we propose DeformPIC, a deformation-based framework for point cloud ICL. Unlike existing approaches that rely on masked reconstruction, DeformPIC learns to deform the query point cloud under task-specific guidance from prompts, enabling explicit geometric reasoning and consistent objectives. Extensive experiments demonstrate that DeformPIC consistently outperforms previous state-of-the-art methods, achieving reductions of 1.6, 1.8, and 4.7 points in average Chamfer Distance on reconstruction, denoising, and registration tasks, respectively. Furthermore, we introduce a new out-of-domain benchmark to evaluate generalization across unseen data distributions, where DeformPIC achieves state-of-the-art performance.

==> sec/3_preliminary.tex <==
\section{Preliminary}
\label{sec:preliminary}

3D Point Cloud In-Context Learning (ICL) is a recently proposed paradigm for point cloud understanding that enables models to perform various tasks given a few demonstrations. Formally, each data example consists of a pair of point clouds $X = (X_i, X_t)$, where $X_i$ denotes the input and $X_t$ the corresponding target. Given a demonstration, referred to as a prompt pair $(P_i, P_t)$ that specifies the task, the model is expected to perform the same task on a query input $Q_i$ and generate the corresponding query target $Q_t$. For example, in a denoising task, both $P_i$ and $Q_i$ represent noisy inputs, while $P_t$ and $Q_t$ are their clean counterparts.

Specifically, Point-In-Context (PIC)~\cite{fang2023PIC} is the first attempt at 3D point cloud ICL, establishing both a solid baseline and a widely adopted evaluation benchmark. Specifically, given prompt pairs $(P_i, P_t)$ and query pair $(Q_i, Q_t)$, PIC uses the Joint Sampling module~\cite{fang2023PIC} to sample aligned central points between prompt data and query data, which forms prompt central points $(C_{P_i}, C_{P_t})$ and query central points $(C_{Q_i}, C_{Q_t})$, respectively. Subsequently, the K-Nearest Neighbors (KNN) algorithm queries the neighborhood points to obtain point patches $(R_{P_i},R_{P_t})$ and $(R_{Q_i},R_{Q_t})$ of these central points.

In the training phase, PIC randomly masks a portion of the target patches $(R_{P_t}, R_{Q_t})$, and replaces these patches with learnable masked tokens. Subsequently, it trains a Transformer~\cite{vaswani2017attention} model to infer the masked content from unmasked target patches and input patches $(R_{P_i}, R_{Q_i})$. PIC adopts Chamfer Distance $L_2$~\cite{fan2017CD} as the training loss, measuring the predicted masked patches $\hat R$ with its corresponding ground truth patches $R$:

\begin{equation}
    \label{eq:cdl2}
    \begin{aligned}
        \mathcal{L}(\hat R, R)=\frac{1}{|\hat R|}\sum_{p\in \hat R}\min_{g\in R}||p-g||_2^2 \\
        +\frac{1}{|R|}\sum_{g\in R}\min_{p\in \hat R}||g-p||_2^2.
    \end{aligned}
\end{equation}

In the inference phase, PIC receives the prompt pair $(P_i, P_t)$ together with the query input point cloud $Q_i$. The to-be-predicted target point cloud $Q_t$ is initialized with the learned masked tokens, which are processed by the Transformer~\cite{vaswani2017attention} together with $(P_i, P_t, Q_i)$ for reconstruction.

It is worth noting that the target point cloud is generated from masked tokens, which contain no geometric information. As a result, the model can only infer the structure and shape from the query input features through the self-attention mechanism. However, such an implicit mechanism often leads to incomplete or inaccurate target geometry. Moreover, there exists a clear training–inference objective mismatch. During training, both the prompt and query targets are randomly masked, and the model learns to recover missing points using visible portions of both targets. Therefore, we propose DeformPIC that reformulates the task as a deformation process and directly transforms the query input toward the target shape under the guidance of prompt examples. In the following section, we describe our DeformPIC in detail.
